Zoom-In-to-Check: Boosting Video Interpolation via Instance-level Discrimination

We propose a light-weight video frame interpolation algorithm. Our key innovation is an instance-level supervision that allows information to be learned from the high-resolution version of similar objects. Our experiment shows that the proposed method can generate state-of-the-art results across different datasets, with fractional computation resources (time and memory) of competing methods. Given two image frames, a cascade network creates an intermediate frame with 1) a flow-warping module that computes coarse bi-directional optical flow and creates an interpolated image via flow-based warping, followed by 2) an image synthesis module to make fine-scale corrections. In the learning stage, object detection proposals are generated on the interpolated image.Lower resolution objects are zoomed into, and the learning algorithms using an adversarial loss trained on high-resolution objects to guide the system towards the instance-level refinement corrects details of object shape and boundaries.

==> tex/exp/table_cityscapes.tex <==
\begin{table}[t!]
\centering
 \begin{tabular}{cccc} 
 \hline\\[-1ex]
  & IE & SSIM & PSNR \\ [0.5ex] 
 \hline \\[-1ex] 
DVF \cite{liu2017voxelflow} & 17.493 & 0.722 & 23.888 \\ 
% final PSNR: 23.888823099114482
% final SSIM: 0.7219372877019415
% final RMSE: 17.492718182086943
SepConv \cite{Niklaus_ICCV_2017} & \textbf{7.852} & \textbf{0.923} &\textbf{30.927}  \\
% final PSNR: 30.927092879189342
% final SSIM: 0.923214404798945
% final RMSE: 7.851976376533508
SuperSloMo \cite{jiang2017superslomo}& $-$ & $-$ & $-$ \\
Ours$_{baseline}$ &9.38  &0.89  &29.31   \\ 
Ours$_{gan}$ & 9.04 & 0.90 & 29.93 \\ 
Ours$_{roigan}$ & 8.39 & \textbf{0.92} & 30.43  \\ 
%  \hline \\[-1ex] 
%   dt=240 ms & IE & SSIM & PSNR \\ [0.5ex] 
%  \hline \\[-1ex] 
% DVF & 25.23 & 0.59 & 20.74  \\ 
% SepConv & \textbf{18.54} & \textbf{0.72} & \textbf{23.67}    \\
% Ours$_{baseline}$ & 19.41 & 0.70 & 23.14 \\ 
% Ours$_{gan}$ & 19.75 & 0.69 & 23.01    \\ 
% Ours$_{roigan}$ & 20.04 & 0.68 & 22.95  \\ 
\hline
\end{tabular}
\caption{Quantitative evaluation of different methods on cityscapes dataset\protect\footnotemark, including Interpolation Error (IE) \cite{Baker2011}, Peak-Signal-To-Noise (PSNR), and Structural-Similarity-Image-Metric (SSIM). Lower IE and higher values of SSIM and PSNR indicate better quality. 
}
\label{tab:cityscapes}
\end{table}
\footnotetext{SuperSloMo \cite{jiang2017superslomo} is not open-sourced so we don't have their results on cityscapes dataset.}

==> tex/exp/table_merge_h.tex <==
\begin{table*}[t!]
\centering
 \begin{tabular}{ccccccc} 
 \hline\\[-1ex]
  & \multicolumn{3}{c}{UCF101 \cite{UCF101}} & \multicolumn{3}{c}{CityScapes \cite{Cordts2016Cityscapes}} \\ [0.5ex] 
  \cline{2-7} \\[-1.5ex] 
  & IE & SSIM & PSNR & IE & SSIM & PSNR \\ [0.5ex] 
 \hline \\[-1ex] 
DVF \cite{liu2017voxelflow} & 11.54 & 0.86 & 29.70 & 17.49 & 0.72 & 23.88 \\ 
SepConv \cite{Niklaus_ICCV_2017} & 11.28 & 0.87 & 30.29 & \textbf{7.85} & \textbf{0.92} &\textbf{30.92}  \\
SuperSloMo \cite{jiang2017superslomo}& \textbf{10.87} & \textbf{0.88} & \textbf{30.48} & $-$ & $-$ & $-$ \\
Ours$_{baseline}$ & 11.23 & \textbf{0.88} & 30.08 & 9.38  &0.89  &29.31   \\ 
Ours$_{gan}$  & 11.66 & 0.87 & 29.85 & 9.04 & 0.90 & 29.93 \\ 
Ours$_{roigan}$ & 11.30 & \textbf{0.88} & 30.14 & 8.03 & \textbf{0.92} & 30.77  \\ 
\hline
\end{tabular}
\caption{Quantitative evaluation of different methods on CityScapes\protect\footnotemark  and UCF101\protect\footnotemark, including Interpolation Error (IE) \cite{Baker2011}, Peak-Signal-To-Noise (PSNR), and Structural-Similarity-Image-Metric (SSIM). Lower IE and higher values of SSIM and PSNR indicate better quality. 
}
\label{tab:merge}
\end{table*}
\footnotetext{SuperSloMo \cite{jiang2017superslomo} is not open-sourced so we don't have their results on CityScapes dataset.}
\footnotetext{We re-run the evaluation on the synthesis images provided by \cite{jiang2017superslomo}.}

==> tex/exp/table_ucf.tex <==
\begin{table}[t!]
\centering
 \begin{tabular}{cccc} 
 \hline\\[-1ex]
   & IE & SSIM & PSNR \\ [0.5ex] 
 \hline \\[-1ex] 
% grayscale w/mask
DVF \cite{liu2017voxelflow}& 11.54 & 0.86 & 29.70\\ 
SepConv \cite{Niklaus_ICCV_2017}& 11.28 & 0.87 & 30.29 \\
SuperSloMo \cite{jiang2017superslomo}& \textbf{10.87} & \textbf{0.88} & \textbf{30.48} \\
Ours$_{baseline}$ & 11.23 & \textbf{0.88} & 30.08\\ 
Ours$_{gan}$ & 11.66 & 0.87 & 29.85 \\
Ours$_{roigan}$ & 11.30 & \textbf{0.88} & 30.14  \\ 
% RGB w/ mask
% DVF & 11.83 & 0.86 & 29.35\\ 
% SepConv & 11.49 & 0.87 & 30.00 \\
% SuperSloMo & 11.08 & 0.88 & 30.20 \\
% Ours$_{baseline}$ & 11.49 & 0.87 & 29.65 \\ 
% Ours$_{gan}$ & - & - & - \\ 
% Ours$_{roigan}$ & \textbf{11.80} & \textbf{0.87} & \textbf{29.42}  \\ 
 \hline 
\end{tabular}
\caption{Quantitative evaluation of different methods on UCF101 dataset \protect\footnotemark, including Interpolation Error (IE) \cite{Baker2011}, Peak-Signal-To-Noise (PSNR), and Structural-Similarity-Image-Metric (SSIM). Lower IE and higher values of SSIM and PSNR indicate better quality. 
%\footnote{We re-run the evaluation on the synthesis images provided by \cite{jiang2017superslomo}.}
}
\label{tab:ucf}
\end{table}
\footnotetext{We re-run the evaluation on the synthesis images provided by \cite{jiang2017superslomo}.}

==> tex/method/algorithm.tex <==
\begin{algorithm}
\caption{ROIGAN}\label{alg:ROIGAN}
\begin{algorithmic}[1]
\Procedure{ROIGAN}{}
\While{$\theta$ has not converged}
    \For{every synthesized and ground truth image pair}
        \For{t = $0$, ..., $n_{critic}$}
            \State Extract all regions of interest $P$, $\Tilde{P}$ and resize them to same shape.
            \For{each update and each layer $l$}
                \State Apply power iteration method to an unnormalized weight $W_l$
                \State Calculate $W_{SN}$ with the spectral norm
                \State Update $W_l$ with SGD on mini-batch dataset $D_M$ with a learning rate $\alpha$
            \EndFor
            \State gw update
            \State w update
        \EndFor
        \State update g0
        \State update 0
   \EndFor
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}
